Rate of Convergence of General Phase Field Equations towards their Homogenized Limit

Over the last few decades, phase-field equations have found increasing applicability in a wide range of mathematical-scientific fields (e.g. geometric PDEs and mean curvature flow, materials science for the study of phase transitions) but also engineering ones (e.g. as a computational tool in chemical engineering for interfacial flow studies). Here, we focus on phase-field equations in strongly heterogeneous materials with perforations such as porous media. To the best of our knowledge, we provide the first derivation of error estimates for fourth order, homogenized, and nonlinear evolution equations. Our fourth order problem induces a slightly lower convergence rate, i.e., $\epsilon^{1/4}$, where $\epsilon$ denotes the material's specific heterogeneity, than established for second-order elliptic problems (e.g. \cite{Zhikov2006}) for the error between the effective macroscopic solution of the (new) upscaled formulation and the solution of the microscopic phase field problem. We hope that our study will motivate new modelling, analytic, and computational perspectives for interfacial transport and phase transformations in strongly heterogeneous environments.

==> acknowledgements2.tex <==
We acknowledge financial support from the Engineering and Physical Sciences
Research Council of the UK through Grants Nos. EP/H034587/1, EP/L027186/1,
EP/L025159/1, EP/L020564/1 and EP/K008595/1 and from the European Research
Council via Advanced Grant No. 247031.


==> ex_shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithmic}
\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

% Declare title and authors, without \thanks
\newcommand{\TheTitle}{An Example Article} 
\newcommand{\TheAuthors}{D. Doe, P. T. Frank, and J. E. Smith}

% Sets running headers as well as PDF title and authors
\headers{\TheTitle}{\TheAuthors}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{{\TheTitle}\thanks{This work was funded by the Fog Research Institute under contract no.~FRI-454.}}

% Authors: full names plus addresses.
\author{
  Dianne Doe\thanks{Imagination Corp., Chicago, IL
    (\email{ddoe@imag.com}, \url{http://www.imag.com/\string~ddoe/}).}
  \and
  Paul T. Frank\thanks{Department of Applied Mathematics, Fictional
    University, Boise, ID (\email{ptfrank@fictional.edu},
    \email{jesmith@fictional.edu}).}
  \and
  Jane E. Smith\footnotemark[3]
}

\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}


%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 

